Hindsight for Foresight: Unsupervised Structured Dynamics Models from Physical Interaction

A key challenge for an agent learning to interact with the world is to reason about physical properties of objects and to foresee their dynamics under the effect of applied forces. In order to scale learning through interaction to many objects and scenes, robots should be able to improve their own performance from real-world experience without requiring human supervision. To this end, we propose a novel approach for modeling the dynamics of a robot's interactions directly from unlabeled 3D point clouds and images. Unlike previous approaches, our method does not require ground-truth data associations provided by a tracker or any pre-trained perception network. To learn from unlabeled real-world interaction data, we enforce consistency of estimated 3D clouds, actions and 2D images with observed ones. Our joint forward and inverse network learns to segment a scene into salient object parts and predicts their 3D motion under the effect of applied actions. Moreover, our object-centric model outputs action-conditioned 3D scene flow, object masks and 2D optical flow as emergent properties. Our extensive evaluation both in simulation and with real-world data demonstrates that our formulation leads to effective, interpretable models that can be used for visuomotor control and planning. Videos, code and dataset are available at http://hind4sight.cs.uni-freiburg.de

==> Makefile <==
PAPER = kuhnerd18iros
EPSFIGURES = 
TIKZFIGURES = #performance
GNUPLOTFIGURESIC =
GNUPLOTFIGURES_EPSFRAG =
TRACKING = 1
PACKAGE =
FAMILY_NAME =
SUBMISSION = aaai18-$(TRACKING)

export BIBINPUTS=.


## Derived variables (don't need to be changed)
EPSFRAGFIGURES = $(GNUPLOTFIGURES_EPSFRAG)
ALLFIGURES = $(EPSFIGURES) $(TIKZFIGURES) $(GNUPLOTFIGURES) $(EPSFRAGFIGURES)
ALLFIGURES_EPS = $(ALLFIGURES:%=figures/%.eps)
ALLFIGURES_PDF = $(ALLFIGURES:%=figures/%.pdf)
ALLGNUPLOTS = $(GNUPLOTFIGURES) $(GNUPLOTFIGURES_EPSFRAG)


## Main targets: paper, pdf, ps, draft, bib, clean, distclean
paper: pdf

$(PAPER).pdf: pdf

$(PAPER).ps: ps

pdf: FORCE $(ALLFIGURES_PDF)
	pdflatex $(PAPER).tex	
	bibtex --min-crossrefs=99 $(PAPER)
	pdflatex $(PAPER).tex	
	pdflatex $(PAPER).tex

ps: FORCE $(ALLFIGURES_EPS)
	latex $(PAPER).tex	
	bibtex --min-crossrefs=99 $(PAPER)
	latex $(PAPER).tex	
	latex $(PAPER).tex
	dvips -Ppdf -G0 -tletter $(PAPER)

draft: FORCE $(ALLFIGURES_PDF)
	pdflatex $(PAPER).tex

bib:
	bibtex --min-crossrefs=99 $(PAPER)

clean:
	rm -f *~ figures/*~ gnuplot/*~ tables/*~ bib/*~ 
	rm -f *.bak figures/*.bak gnuplot/*.bak tables/*.bak bib/*.bak
	rm -f *.new figures/*.new gnuplot/*.new tables/*.new bib/*.new
	rm -rf auto tables/auto figures/auto
	rm -f $(PAPER).aux $(PAPER).bbl $(PAPER).blg
	rm -f $(PAPER).dvi $(PAPER).log $(PAPER).ps $(PAPER).pdf

distclean: clean
	rm -f $(PAPER).pdf

FORCE:

.PHONY: paper pdf ps draft bib clean distclean FORCE


## Rules related to version for initial submission
submission: $(SUBMISSION).pdf

$(SUBMISSION).pdf: FORCE $(ALLFIGURES_EPS)
	cp $(PAPER).tex $(SUBMISSION).tex
	latex $(SUBMISSION).tex
	bibtex --min-crossrefs=99 $(SUBMISSION)
	latex $(SUBMISSION).tex
	latex $(SUBMISSION).tex
	latex $(SUBMISSION).tex
	dvips -Ppdf -G0 -tletter $(SUBMISSION).dvi
	ps2pdf -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 \
	  -dMaxSubsetPct=0 -dSubsetFonts=false -dEmbedAllFonts=true \
	  -sPAPERSIZE=letter $(SUBMISSION).ps

submission-clean:
	rm -f $(SUBMISSION).aux $(SUBMISSION).bbl $(SUBMISSION).blg
	rm -f $(SUBMISSION).dvi $(SUBMISSION).log $(SUBMISSION).ps
	rm -f $(SUBMISSION).tex $(SUBMISSION).pdf

clean: submission-clean
.PHONY: submission submission-clean


## Rules related to camera-ready copy submission package
package: FORCE
	../scripts/aaai/make-aaai-package $(PAPER) $(PACKAGE) $(FAMILY_NAME)

package-clean:
	rm -f $(FAMILY_NAME).log
	rm -f $(PACKAGE).tgz 
	rm -rf $(PACKAGE)

clean: package-clean
.PHONY: package package-clean


## Rules related to EPS and PDF figures
$(ALLFIGURES_PDF): %.pdf: %.eps
	epstopdf --outfile=$*.pdf $*.eps

epsfig-clean:
	rm -f $(ALLFIGURES_EPS) $(ALLFIGURES_PDF)

clean: epsfig-clean
.PHONY: epsfig-clean


## Rules related to figures that need to be processed with epsfrag.py
epsfrag:
	mkdir epsfrag

$(EPSFRAGFIGURES:%=epsfrag/%.epsfrag.eps): epsfrag
$(EPSFRAGFIGURES:%=epsfrag/%.frag): epsfrag

$(EPSFRAGFIGURES:%=epsfrag/%.eps): epsfrag/%.eps: epsfrag/%.epsfrag.eps epsfrag/%.frag
	cd epsfrag && ../../scripts/epsfrag.py $*.epsfrag.eps $*.frag $*.eps

$(EPSFRAGFIGURES:%=figures/%.eps): figures/%.eps: epsfrag/%.eps
	cp $< $@

epsfrag-clean:
	rm -f $(EPSFRAGFIGURES:%=epsfrag/%.epsfrag.eps)
	rm -f $(EPSFRAGFIGURES:%=epsfrag/%.frag)
	rm -f $(EPSFRAGFIGURES:%=epsfrag/%.aux)
	rm -f $(EPSFRAGFIGURES:%=epsfrag/%.dvi)
	rm -f $(EPSFRAGFIGURES:%=epsfrag/%.log)
	rm -f $(EPSFRAGFIGURES:%=epsfrag/%.tex)
	rm -f $(EPSFRAGFIGURES:%=epsfrag/%.ps)
	rm -f $(EPSFRAGFIGURES:%=epsfrag/%.eps)
	if [ -d epsfrag ]; then rmdir --ignore-fail-on-non-empty epsfrag; fi

clean: epsfrag-clean
.PHONY: epsfrag-clean


## Rules related to gnuplot

## NOTE on dependencies:
## This rebuilds all gnuplots as soon as a single *.data file has been
## changed. It would be preferable to only rebuild if a data file
## related to the plot has been changed, but this doesn't seem to be
## possible to do. I tried $(wildcard gnuplot/%*.data), but make
## doesn't seem to support this. Since plot data only changes
## infrequently, the extra effort shouldn't be too bad.

$(ALLGNUPLOTS:%=gnuplot/%.eps): gnuplot/%.eps: $(wildcard gnuplot/*.data)

$(ALLGNUPLOTS:%=gnuplot/%.eps): gnuplot/%.eps: gnuplot/%.gp
	cd gnuplot && gnuplot $*.gp

$(GNUPLOTFIGURES_EPSFRAG:%=epsfrag/%.epsfrag.eps): epsfrag/%.epsfrag.eps: gnuplot/%.eps
	cp $< $@

$(GNUPLOTFIGURES_EPSFRAG:%=epsfrag/%.frag): epsfrag/%.frag: gnuplot/%.frag
	cp $< $@

$(GNUPLOTFIGURES:%=figures/%.eps): figures/%.eps: gnuplot/%.eps
	cp $< $@

gnuplot-clean:
	rm -f gnuplot/*~
	rm -f $(ALLGNUPLOTS:%=gnuplot/%.eps)
	rm -f $(ALLGNUPLOTS:%=gnuplot/%.png)

clean: gnuplot-clean
.PHONY: gnuplot-clean


## Rules related to TikZ figures

## NOTE: Using dvips -E (and thus avoiding ps2epsi) gets the bounding
##       box wrong.
$(TIKZFIGURES:%=figures/%.eps): figures/%.eps: figures/%.tex
	cd figures && latex $*.tex
	cd figures && dvips -P pdf -o $*.ps $*.dvi
	cd figures && ps2epsi $*.ps $*.eps

tikz-clean:
	rm -f $(TIKZFIGURES:%=figures/%.aux)
	rm -f $(TIKZFIGURES:%=figures/%.dvi)
	rm -f $(TIKZFIGURES:%=figures/%.log)
	rm -f $(TIKZFIGURES:%=figures/%.ps)

clean: tikz-clean
.PHONY: tikz-clean


==> figures/title.tex <==
\begin{tikzpicture}
\node[anchor=north west,inner sep=0] (image) at (0,5.4) {\includegraphics[width=1\columnwidth]{figures/cover_tmp.png}};
\end{tikzpicture}


